PiXi: Password Inspiration by Exploring Information

Passwords, a first line of defense against unauthorized access, must be secure and memorable. However, people often struggle to create secure passwords they can recall. To address this problem, we design Password inspiration by eXploring information (PiXi), a novel approach to nudge users towards creating secure passwords. PiXi is the first of its kind that employs a password creation nudge to support users in the task of generating a unique secure password themselves. PiXi prompts users to explore unusual information right before creating a password, to shake them out of their typical habits and thought processes, and to inspire them to create unique (and therefore stronger) passwords. PiXi's design aims to create an engaging, interactive, and effective nudge to improve secure password creation. We conducted a user study ($N=238$) to compare the efficacy of PiXi to typical password creation. Our findings indicate that PiXi's nudges do influence users' password choices such that passwords are significantly longer and more secure (less predictable and guessable).

==> Background.tex <==
\section{Related Work} \label{bg}
We describe nudging using cybersecurity examples in Section \ref{bg:nudging}, then review literature on nudges at the time of password creation in Section \ref{bg:pwdcreation}.  

\subsection{Nudging} \label{bg:nudging}
% Nudging is the core, so we first talk about the nudge and how it affect users' decisions
Nudging is a promising strategy to encourage people to make better or more desirable choices.  Examples of nudging include framing, priming, and visualizations \cite{caraban201923}. Thaler and Sunstein \cite{thaler2008nudge} defined nudges as ``any aspect of the choice architecture that alters people's behavior in a predictable way without forbidding any options or significantly changing their economic incentives''. Nudging has been applied in a variety of domains including education \cite{breman2011give}, ethics \cite{bazerman2012behavioral}, social context \cite{johnson2003defaults}, health \cite{quigley2013nudging,milkman2011using,vanepps2016calorie},  finance \cite{karlan2016getting,cai2020nudging,carroll2009optimal,thaler2004save,breman2011give}, energy savings \cite{camilleri2014metric,costa2013energy}, privacy \cite{acquisti2017nudges}, and security \cite{collier2018nudge}.  Nudging studies have proved that nudges can successfully influence people's decisions by minor and inexpensive interventions \cite{dijksterhuis2000relation}. Hansen et al. \cite{hansen2013nudge} redefined nudges according to the two human thinking forms (System 1 \& System 2) and the transparency proposed by Kahneman's framework \cite{kahneman2003maps,thinking2011fast}. They expanded the human dual process theories which contains two modes of thinking, System 1 (automatic mind) and System 2 (reflective mind) into 4 categories: 1) System 1, manipulating behavior (e.g., changing the order of WiFi list to promote stronger WiFi), 2) System 1, influencing behavior (e.g., painting illusions of speed bumps on streets to encourage careful driving), 3) System 2, manipulating choice (e.g., offering unattractive options to the set of choices to make the certain choice more attractive), 4) System 2, prompting reflective choice (e.g. providing real-time feedback to evaluate password strength). Humans prefer to think and make decisions via autonomic processing with minimum effort, which occasionally leads to making unwise decisions.

%Then we introduce some methods to improve password security using nudging
Throughout the years, computer security experts and administrators have been investigating nudges to encourage secure behaviors \cite{zimmermann2021nudge}. Seitz et al. \cite{seitz2016influencing} sought to persuade users to pick stronger passwords by providing multiple password suggestions using the decoy effect, which uses one unpleasant choice as a decoy to make the other option seem more appealing. The study's findings concluded that an effective nudge should provide only the best suggestion with more transparent and perceivable explanation. Von Zezschwitz et al. \cite{von2016quantifying} tried to enhance the effectively utilized password space for Android unlock patterns by presenting background visuals and animations throughout the password formation process. The experimental study result indicated that their nudge had very limited influence when a substantial proportion of users were unaware or confused about the nudge, such as background images or animations changing, and the existence of ``counter-nudges'' caused by the user's own strong habits. Similarly, Briggs et al. \cite{briggs2014nudging} changes order of color and menu to encourage users to choose a more secure Wi-Fi. The authors indicated that the nudge effect is reduced when users have different decision-making styles, and personal preferences have significant influence on security decisions.


%We also introduce "Hybrid Nudge", an upgrate version (textual+graphical) of simple nudging (textual), PiXi is using hybird nudge as the (structure).
%\subsection{Hybrid Nudge}

According to Hansen et al.'s work \cite{hansen2016definition}, Renaud et al. \cite{renaud2019nudging} defined simple nudge is defined as ``a simple intervention that using system 1 (automatic mind) only''. However, in many real-world circumstances, simple nudges may not handle the issues of pre-existing habitual behaviors, or strong personal preferences when it delivers messages mainly through System 1 without supporting System 2 \cite{sunstein2017nudges}. In order to address the above issues, Zimmermann et al. \cite{zimmermann2021nudge} proposed hybrid nudge, which is defined as ``a more comprehensive intervention combining a simple nudge and information provision involving both systems''. Hansen et al.'s \cite{hansen2016definition} examined the effectiveness of simple nudges and hybrid nudges in promoting the use of strong passwords. They reported that the simple nudge has little influence on the strength of a password, and cannot offset habitual password choice behaviors. By comparison, the hybrid nudge reduced the uncertainty, highlighted the benefits, and simplified the internal cost–benefit analysis when each intervention plays a significant role, leading to the hybrid nudge as a whole achieving an outstanding outcome. 

%Then we introduce "Personalized Nudge", PiXi is using Personalized Nudge as the (output)
%\subsection{Personalized Nudge}

The majority of nudges we see today adhere to the ``one-size-fits-all'' approach and are built for the 'average user' \cite{carroll2009optimal,peer2020nudge,yeung2017hypernudge}. While a one-size-fits-all nudge is easy to implement, it is inefficient to protect most users away from dangerous behaviors or even have a negative impact on some users \cite{thunstrom2018nudges} when users are significantly diverse in terms of cognitive styles, educational backgrounds, expertise, or personal preferences. The first concept of personalized nudge was proposed by Sunstein el at. \cite{sunstein2013impersonal}. He argues that personalized nudge would “reduce the problems posed by one-size-fits-all approaches” if it collects enough data. Then Thaler et al. \cite{thaler2013smarter} introduced ``choice engines'', which use different kinds of heterogeneity data to generate personalized recommendations. Mills et al. \cite{mills2022personalized} summarized prior research and offered the choice and delivery personalization framework. ``choice personalization uses personal information to determine which choice to nudge the decision-maker towards, and delivery personalization uses personal information to determine which nudging method to apply to the decision-maker. Peer et al. \cite{peer2020nudge} explored the delivery personalization in password creation processes, using individual differences in decision-making styles to determine the best online password nudge for each user. They found that personalized nudges provided more promising results, increasing nudges’ efficacy up to four times compared to one-size-fits-all nudges.

%This section is optional. However, PiXi is using very similar technique to influencing users (choosing keywords)

\subsection{Password Creation Nudges} \label{bg:pwdcreation}

Nudging techniques have been employed, with varying degrees of success, to enhance the security of both graphical and text passwords. Throughout this review, we categorize the types of nudges employed using the framework of Caraban et al. \cite{caraban201923}.  As part of this review, we identified a number of papers previously not considered/named as nudges in other surveys (e.g., \cite{BDAS,vonZezschwitz2016,ThorpePriming,PARISH2021102913,Katsini,macrae2016strategies,Houshmand}.  

\subsubsection{Nudges for Graphical Passwords}

%Start with a brief sentence defining graphical passwords and reference the Biddle et al. survey (ACM Survey paper).
Graphical passwords are a type of authentication that involve remembering picture(s) or parts of pictures instead of a word. Graphical passwords can be categorized as\cite{GraphicalPasswords} 1) Pure-recall, requiring users to draw a secret using images or patterns (e.g., Draw-A-Secret(DAS) \cite{DAS}, BDAS \cite{BDAS}) 2) Cued-recall(e.g., PassPoints \cite{PassPoints}, CCP \cite{CCP}, and GeoPass \cite{GeoPass,thorpe2007human}) require users remember and target specific locations within an image. 3) Recognition-based (e.g., PassFaces \cite{passfaces}, Story \cite{Story}, and VIP \cite{bicakci2009graphical}) asks users to memorize a portfolio of images during password creation, and then recognize their images from among decoys to log in. To improve graphical password security, many nudging techniques have been proposed and evaluated. 

Background Draw-A-Secret (BDAS)\cite{BDAS} may have been the first attempt to nudge users away from typical patterns during graphical password selection. It presents users with a background image, on which they need to draw their graphical password. Its background image should evoke the ``salience bias", which refers to the fact that users are more likely to focus on information that is more prominent.  The visual element of the background image aims to facilitate the creation of different graphical passwords than if the background image was not present. It can also be considered as a reinforce (subliminal priming) nudge. Findings indicated that BDAS did significantly increase indicators associated with password strength, (e.g., stroke count and length).  Zezschwitz et al. \cite{vonZezschwitz2016} used nudging to help users create stronger patterns on Android mobile devices. They designed a variation based on background images (similar to BDAS, but using the Android pattern as the basis instead of Draw-A-Secret). %While the lab-based evaluation of the system was very promising, the field study involving 496 users on MTurk platform yielded only small effects. 
The study results revealed that users selected a more diverse set of longer patterns when background images were present.

Persuasive Cued Click Points (PCCP) \cite{PCCP} can be considered a facilitate (suggesting alternatives) nudge where users have to select from a point within a randomly positioned view-port (all other options are not available). If desired, they can use the shuffle button to change the view-port to another random location. The system was found to have minimal usability impact compared to other cued-recall systems; however, it does hamper a user's free choice if they wish to select a specific point --- in this case the user would need to ``shuffle" many times in the hopes of being able to select their desired choice. To implement PCCP as a true nudge, it would need to permit a user to override the view-port to select any point of their choosing.  

A number of systems\cite{ThorpePriming,PARISH2021102913,Katsini} based on PassPoints \cite{PassPoints} can be considered a facilitate (hiding) and reinforce (subliminal priming) nudge. They aim to nudge users away from common patterns by presenting the background image differently at the password creation.  Image presentations reveal the background image slowly so the user will perceive it differently.  Since these nudges temporarily hide certain options (making them harder to reach), it can be categorized as a facilitate (hiding) nudge. As some parts of the image will be initially revealed and exposed to the user for a longer time, it also involves a reinforce (subliminal priming) nudge. Studies found simple image presentations produced different distributions in user-chosen click points, suggesting that it can significantly impact user's choice without reducing usability \cite{ThorpePriming,PARISH2021102913}. % and the majority (80\%) of participants had no problem with the image presentation.
Presenting the image such that it reveals starting from the least salient parts, ending with the most salient parts has been found to have different impacts on users password strength depends on users' cognitive style and background image\cite{Katsini}. %Field Independents created stronger passwords using more complex background images. In contrast, Field Dependents created stronger passwords using a simpler background image.  

%Katsini et al. \cite{Katsini} examined image presentations effect to investigate if the complexity of background images can affect password strength. The authors conducted 2 studies with 36 participants from the university, where participants use a cued-recall graphical authentication scheme with different images. The results suggested that the image complexity has a strong correlation to users passwords strength, users with complex images (include more saliency points) can create more secure passwords.
% image presentations that revealed the image starting from the least salient parts, showing the most salient parts last
%There are 4 images in total. 1 original simple image (sky + small airplane), 1 orignial complex image (many ppl in a room, chatting with coffee and many small objects in the room). 1 mooney image of the simple image, 1 mooney image of the complex image. [FD(field-dependent), FI(field-indpendent), there is no explaination about what are FD and FI is..i'm trying to google it]
%Regarding the simple image, the FDs were not affected by our mechanism, as their passwords were already strong. Sim-ilarly, to the case of the simple image of the exploratory study, they used the saliency points as reference points for drawing their gestures. On the other hand, FIs created stronger passwords compared to those created by the FIs in the exploratory study. Compared to the exploratory study, FIs extended the active drawing area of their gestures and used more combinations (e.g., they created passwords in-cluding all three gestures more often). As a result, they cre-ated stronger passwords than the passwords created by FIs when the saliency mask mechanism was not active (explora-tory study). Despite that the strength of the passwords cre-ated by the FIs increased, they were still less strong when compared to those created by the FDs, as FIs focused again on the main parts of the airplane (i.e. primary point of inter-est), such as the airframe and the wings.
%Regarding the complex image, both FDs and FIs created stronger passwords compared to those of the complex image of the exploratory study. FDs faced difficulties with pro-cessing visual complex scenes, and our mechanism allowed them to process more visual information because it was dis-played gradually to them within 20 seconds. Hence, they had more time to conceptualize the context of the image and spot simple objects (e.g., notebook, pot), which they used to draw their gestures on. Likewise, our saliency mask mechanism helped FIs to identify various objects in the scene (e.g., pot on the self, ceiling lights), which were not among the primary attention points. Due to their skill to conceptualize details fast, they used such items to form their graphical password.


%Consider whether this, as well as the PTP and PassMod systems could be considered "Facilitate-Hiding" nudges.  Eventually, if they shuffle enough, would they reach the whole possible set of items they could choose? 
%I think PTP and PassMod systems could be considered "Facilitate-Hiding" nudges. I have checked the paper and I believe users can reach all the items/points with enough shuffle click.

 
%Chiasson et al. introduced Persuasive Cued Click Points (PCCP) as an upgraded version of CCP, which addresses the issues related to hot-spot points during password creation with persuasive features. In PCCP, users are not allowed to freely choose their desired click-points but have to select from a click-point within a random position view-port. They can use the shuffle button to change the view-port to another random location. The researchers conducted a study to compare the performance of PCCP with CCP, PassPoints (PP), and the control condition. The study found that PCCP had similar success rates (94\%, 98\%, 96\%) and login times (18s, 12s, 10s) to the other schemes. However, the usability of PCCP was not evaluated as the researchers did not provide any information regarding participants' preferences for PCCP compared to CCP or other systems.

While these nudging results are interesting, the market has yet to see many viable graphical password products due to deployability issues such as cost and accessibility \cite{6234436}. As a result, there is more interest in developing effective nudges for widely-deployed text password systems.


\subsubsection{Text Password Nudges}
The most straightforward way to nudge strong password selection is to suggest a random password to the user. This is a form of facilitate (default) nudge, if implemented so the user has a choice to accept the random password or not. 
 However, memorability is a significant problem for system-assigned random passwords \cite{1341406}. %Attempts have been made to help improve memorability of secure system-assigned passwords, e.g. through passphrases \cite{Shay}, however they unfortunately were not effective.  
 Password managers can help users remember a random password, but many users still hesitate to adopt them \cite{281272}. Even for those users who are successfully nudged to choose a random password and store it in a password manager, it is recommended to avoid using password managers for sensitive accounts (e.g., email, financial, workplace, etc.) \cite{CanadianGovt}. For these reasons, finding other ways to nudge users towards creating secure passwords remains of interest.     

One way to nudge users towards creating stronger text passwords is through password meters, which employ a confront (creating friction) nudge to provide real-time feedback on password strength. The hope is that its feedback will nudge users to revise their passwords to be stronger. Ur et al. \cite{180204} designed and examined 14 password meters, each of them using different visual effects and nudge techniques. 
%The study had 2 sessions, involving 2931 Amazon MTurk participants for Session \#1 and 2,016 participants returned for Session \#2. 
The results show that some password meters with visually appealing interfaces and strict prompts can significantly enhance security against a strong adversary. %When no meter was used, 46.7\% of passwords were cracked, compared with 39.4\% in the baseline (an insignificant improvement). However, there was a significant improvement in the half-score (26.3\% cracked) and third-score groups, where 26.3\% and 27.9\% were cracked respectively. The half-score and third-score groups used visually appealing interfaces and stricter requirements for security measurements (half-score halving the score and third-score giving one-third of the score of the baseline system respectively). 
The finding indicates that strict nudge prompts can be more effective at creating friction. Unfortunately, many participants of these successful meters (38-39\%) %in half-score and 39\% in one third-score 
found the meter annoying. One possible reason is that password meter nudges create friction, but do not facilitate users in coming up with an acceptable secure password.  

%2
%Password managers are a popular technique that can help alleviate the burden of managing multiple accounts and passwords for users. These tools make it easy to handle multiple accounts, and password generators can create strong and random passwords that fit any password policy. Zibaei et al. \cite{Password_Meter_1} conducted a study on the effectiveness of nudges in encouraging users to adopt randomly generated passwords in Chrome, Firefox, and Safari. The researchers found that users in Safari (61\%) were more likely to accept randomly generated passwords when prompted by a better nudge browser with attractive and interesting visual effects. However, strict password policies may not be helpful in encouraging users to accept these passwords. While password managers can be helpful, users still need to create a strong and memorable master password for their password manager, which can be challenging. If the master password is lost, all other passwords stored in the password manager become inaccessible, rendering their security measures meaningless. Government of Canada\footnote{https://www.getcybersafe.gc.ca/en/secure-your-accounts/password-managers\#defn-password} has suggested that passwords for sensitive accounts like Email and financial should not be stored in password managers. Therefore, users must find a way to create a strong master password that they can remember.

Other approaches employ a facilitate (suggesting alternatives) nudge that suggests modifications to the initial password to make it secure. These systems could be implemented as a nudge, where the user can dismiss the suggested modification if desired, but the following implementations only provided the option to ``shuffle" to generate a new suggestion if they were unhappy with the one the system provided.  %We review them under the assumption they can be implemented as a suggestion which the user could reject and choose their own password if desired. 
%3
In Persuasive Text Passwords (PTP)\cite{forget2008improving}, after a user creates a password, random characters are added at random positions to increase the complexity of the password. The user can then use a shuffle button to repeat this process until they are satisfied with the final password. Initial memory tests (in the same session as creation) showed promise, but password creation time was significantly increased as users often use the shuffle button (18 times on average) before finding an acceptable system-suggested password. %While users believed PTP helped them create more secure passwords, they didn't find them easier to create, and had generally longer create, confirm, and login times. 
Houshmand et al.\ \cite{Houshmand} proposed that the suggestions be built using probabilistic context free grammars.  Both PTP and Houshmand's modification systems were found to be vulnerable to Guided Brute Force attacks \cite{schmidt_acsac13}.
 %they found these passwords more difficult to create.  
%4
%Shayetal. \cite{Shay} explored the possibility of using system-assigned random passphrases instead of system-assigned passwords with random characters, by encouraging users to imagine a scene that find connection among each passphrase, and re-type those passphrases as their passwords when they need to login. However, the results of the user study were not positive. The study found that the usability and memorability of system-assigned random passphrases did not improve significantly compared to system-assigned passwords with random characters. Only 48.5\% of participants were able to recall the passphrases after 2-3 days, indicating that they were not significantly easier to remember. 
%5
In PassMod \cite{macrae2016strategies}, the suggestions are built using semantic grammar generation algorithms to extract weak words from user input and replace them with strong words. A small feasibility study indicates PassMod successfully strengthened participants' passwords and 74\% of users could remember their suggested passwords after 7-8 days. Most participants (71.4\%) reported satisfaction with the system suggestions. While the results were promising, the study only involved 43 student participants, and had no control group, so further study is needed to determine its efficacy.


% @Tony: this below paper still needs more details.  There's not enough here to understand what the nudge is, how the user interacts with it, etc.  Please add.

%Do we still need this part.. This hybrid nudge was a subsection of nudging, the purpose of it is to prove that using one or more nudges in a system (hybrid nudge) is more effective than a system with only 1 nudge.
%Renaud et al. \cite{renaud2019nudging} investigated the effectiveness of hybrid nudges compared to simple nudges in improving password strength during password creation. The researchers conducted three user studies to investigate 1) if simple nudge can affect users password choices? 2) if a hybrid nudge is more effective than a simple nudge?. The first study invited 497 participants. The system involves 5 different simple nudges, and each of them present different information to users before creating passwords. Two of them show a graph with minor wording changes related to password life circles, two of them provide password meters (with minor wording changes as well) (confront (friction) nudge) and the above graph, and one provides a sentence (subliminal priming nudge). All the above nudges are displayed on the top of the password creation input box. Comparing those 5 simple nudges to the control condition (standard registration without nudges), they found that the simple nudges did not significantly impact the password strength. The second study invited 737 participants. It includes all nudges from study 1 and a new simple nudge using a single image (An eye is watching you) only. The result was the same as the first study. The third user study, all participants (672 participants) were assigned to the same experimental condition to evaluated the effectiveness of a hybrid nudge. The hybrid nudge consists of 3 parts. A simple nudge using an image to encourage participants pay attention the the massage. An incentive or (confront (friction) nudge) nudge provides a real-time feedback about their passwords-strength in lifespan format, and a reminder to remind users every time they log in how much longer their password is valid. The results shows that the hybrid nudge improved both password length (study1\_mean=9.59, study2\_mean=10.02, study3\_mean=11.35) and strength (study1\_mean=1.64, study2\_mean=1.8,study3\_mean =2.66) using ZXCVBN as measured with the same score metric used in the previous studies. 


%Overall. in order to mitigate text and graphical passwords limitations, and integrate graphical passwords techniques and nudges on 63 text password authentication schemes, we proposed PiXi, which employes graphical and textual nudges, with persuasive approach to encourage users choose strong passwords. 

%It indicated Password meters do not provide any ideas for users when they create passwords, and they are limited in their ability to guide users before they choose a password. Users have to spend extra time and effort to create, modify, and adapt their passwords to comply with specific password policies from password meters.

In summary, the existing approaches to nudge stronger passwords are either (a) default nudges to use a randomly generated password (typically employed as a nudge in password managers \cite{281272}), (b) confront (friction) nudges that aim to increase user's awareness of their chosen password's weakness, with no facilitation in coming up with a new password (e.g. password meters \cite{ur2015measuring}), and (c) facilitate (suggesting alternatives) nudges that suggest modifications to a user's initially weak password to make it secure (e.g., \cite{forget2008improving,macrae2016strategies,Houshmand}.   
 Our approach with PiXi is entirely different than previous text password nudges; we aim to facilitate user's password creation without suggesting alternatives, but instead using the following set of nudges immediately prior to password creation: (i) facilitate (positioning and suggesting alternatives) to help users explore an unusual path (and set of selections) through the PiXi system, (ii) confront (throttling mindless activity) to ensure users consider their PiXi selections, and (iii) reinforce (subliminal priming) to make the user's PiXi selections more prominent and easily accessible at the time the user is attempting to conceive a new password.  The goal of this combination of nudges is to create an engaging, interactive, and effective nudge to impact password creation.

==> Discussions.tex <==
\begin{comment}
\section{Discussions} \label{ds}
In this section, we discuss limitations and promising directions for further improvements and study.

\subsection{Future Work: Enhancing PiXi} 
PiXi presently only offers three categories. In future work, we suggest the addition and study of additional categories to provide users with a broader set of unique paths/nudges through the system. Additional categories of interest include music/songs, videos, maps, news, or blog posts. 


%\subsection{Future Work: Studies}

\subsection{Limitations}
Our study used Amazon MTurk, which we found to have a notable amount of noise. While we did our best to fairly catch noise and remove from our dataset, it is possible we couldn't catch and filter all noisy data. The implications of such noise on our data is that differences between conditions cannot be detected (e.g., relating to SUS data). However, since the noise should be consistent between each group, any statistically significant finding should be reliable. Future studies should focus on other populations or enhanced methods to filter noise on MTurk. Such future studies should also focus on long-term recall rates, and related login times over successive logins. It would also be interesting to study whether a shortened version of the PiXi system (e.g., involving only one keyword) could be equally effective at nudging users towards choosing secure passwords.

\end{comment}

%\subsection{Optimized Search Function}
%The majority of participants choose to use default items over searching. In order to make their passwords more difficult to crack, we expect that the system can nudge participants to look for or choose such uncommon elements. Use of extra textual or graphical cues before or during decision-making is one potential option. Another option is to automatically conceal well-known, simple-to-guess things. Real-time dynamic lists for well-liked goods and keywords should be produced by the system. The system should display the only things that are not included in the lists before default items or search results are shown.

%\subsection{Amazon MTurk Reliability Concerns}

%The participants we selected from Amazon Mechanical Turk are all from the United States and have a minimum approval rate of 95\%. Although high approval rate indicates they are "pay attention" to tasks from Amazon MTurk perspective, every situation has a flip side. In one hand, when eligible Amazon MTurk participants come from the same country, population diversity is reduced. In another hand, participants with high approve rates have "over" sufficient experience to do tasks, which means they may primarily focus on how to quickly complete tasks to get incentives instead of paying attention to system details or think why they made such decisions, and such negative activities significant impact our user study and other researchers as well \cite{281272}. In the future, we intend to conduct further in-person user studies involves different kinds of participants.

%\subsection{Increasing Options}
%PiXi/PiXi-Hints presently only offers three categories due to the limited amount of time and effort, and one category, music, is still in the process of being developed. We are going to add other categories in order to provide participants with more comprehensive resources and to encourage them to select a range of keywords in a number of different media, such as brief videos, locations through maps, text and images in breaking news, blog posts, or audio recordings. These can all be found on our website.

%\subsection{Improving APIs Rate-limit and Reliability.}
%Currently, the PiXi/PiXi-Hints is using 3 free-to-use APIs, two of which (Unsplash and TMDB) are in demo mode and have relatively low rate limits, which means they will cease to function for a period of time if an abnormally high volume of queries occurs in a short period of time. Additionally, if they are unavailable (either for maintenance or due to cyber attacks), availability of PiXi will be greatly impacted. To overcome the aforementioned concerns, we intend to apply for production licenses for the future research, which entitles us to higher rate limits. Another option is to develop our own APIs, which may takes a long time and effort.

%\subsection{Further Developments for Novel Authentication Frameworks.}
%PiXi/PiXi-Hints was created to motivate people to create more secure and memorable textual passwords. In other words, PiXi continues to support the traditional text password authentication framework, which has well-known issues with memorability and susceptibility. In future study, we will investigate PiXi variants that might be used in replacement of password authentication. For instance, an variation that enables participants login by clicking a sequence of chosen keywords form a category without typing a password.

%\subsection{Memorability Evaluation}
%Although we have already conducted a two-session user study to evaluate the effectiveness of PiXi and PiXi-Hints in generating secure and memorable passwords, we encountered issues with the Amazon MTurk robots that prevented us from using the data collected in the second session. Additionally, we were unable to conduct a memorability evaluation due to these issues. Therefore, we plan to conduct another in-person user study in the future to overcome these limitations and collect more reliable data. This future study will allow us to evaluate the memorability of passwords generated by our proposed system and further investigate the effectiveness of personalized nudges in encouraging users to create stronger and more memorable passwords.

%\subsection{Potential Attacks From The Pixi Password Reset Function}
%Currently, each user's keywords and their related footprints are tracked by the PiXi system.
%The password reset function makes the first keyword (hint) and cover used to create an account public, providing opportunities for attack by known adversaries. Depending on the success rate of the post-hint, this function operates [well or poorly]. If the attackers get to get the victim's email address, they could use it to create some dictionaries to try to guess the password. Attackers may determine from the cover which category the victim chose through observation or the use of image search engines (Ex. Google or TinEye Reverse Image Search). Attackers may analyse the trending keywords or extract all the words (from books and movies) or tags (from images) from the selected item after receiving the category and the initial clue, and then create attack dictionaries.

==> EasyGuess.tex <==
\begin{table}[h]
\begin{tabular}{llll}
\hline
\multicolumn{4}{c}{\textbf{Easy-Guess Password List}} \\ \hline
\multicolumn{1}{l|}{} & \textbf{Control} & \textbf{PiXi} & \textbf{PiXi-Hints} \\ \hline
\multicolumn{1}{l|}{\textbf{1}} & 19761976 & 147258369 & 789456123 \\ \hline
\multicolumn{1}{l|}{\textbf{2}} & 54545454 & Qwerty12345 & magazine \\ \hline
\multicolumn{1}{l|}{\textbf{3}} & 14514500 & speaker1 & DRINKING \\ \hline
\multicolumn{1}{l|}{\textbf{4}} & background & 12345678\$\$ & temppass \\ \hline
\multicolumn{1}{l|}{\textbf{5}} & butterfly & abcdefg123 & john1234 \\ \hline
\end{tabular}
\caption{The top 5 weakness password across the 3 conditions.}
\label{tab:easy_guess}
\end{table}

==> Q5Result.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll} 
\hline
\textbf{N} & \textbf{\textbf{Test Statistic}} & \textbf{\textbf{Degree Of Freedom}} & \textbf{\textbf{P}}  \\ 
\hline
238               & 56.575                           & 2                                   & .001                       \\
\hline
\end{tabular}
\caption{Summary of Q5-Independent-samples Kruskal-Wallis test.}
\label{tab:q5-result}
\end{table}

==> SUSGuidline.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lll}
\hline
\textbf{SUS Score} & \textbf{Grade} & \textbf{Adjective Rating} \\ \hline
\textgreater 80.3  & A              & Excellent                 \\
68 – 80.3          & B              & Good                      \\
68                 & C              & Okay                      \\
51 – 68            & D              & Poor                      \\
\textless 51       & F              & Awful                     \\ \hline
\end{tabular}
\caption{General guideline on the interpretation of SUS score.}
\label{tab:sus-guidline}
\end{table}

==> SUSScore.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
               & \textbf{Mean} & \textbf{N} & \textbf{Std. Deviation} \\ \hline
\textbf{Control}     & 56.6            & 71         & 13.28                      \\
\textbf{PiXi}     & 54.48            & 83         & 11.93                      \\
\textbf{PiXi-Hints}    & 56.68           & 84        & 11.49                     \\
\textbf{Total} & 56            & 238         & 12.3                      \\ \hline
\end{tabular}
\caption{Mean SUS score across the three conditions.}
\label{tab:mean-sus}
\end{table}

==> ZXCVBN_Result.tex <==
\begin{table}[]
\begin{tabular}{llll}
\hline
 & \textbf{\begin{tabular}[c]{@{}l@{}}\textless{}=10\textasciicircum{}6\\ (online)\end{tabular}} & \textbf{10\textasciicircum{}6 $\sim$10\textasciicircum{}14} & \textbf{\begin{tabular}[c]{@{}l@{}}\textgreater{}=10\textasciicircum{}14\\ (offline)\end{tabular}} \\ \hline
\textbf{Control} & 43.7\% & 56.3\% & 0\% \\
\textbf{PiXi} & 32.5\% & 66.4\% & 1.1\% \\
\textbf{PiXi-Hints} & 32.4\% & 64.9\% & 2.7\% \\ \hline
\end{tabular}
\caption{Password guesses distribution using ZXCVBN.}
\label{tab:ZXCVBN_Guesses}
\end{table}

==> bookList.tex <==
\begin{table*}[b]
\centering
\begin{tabular}{ll|ll}
\hline
1  & The Gathering Storm - Chapter One               & 45 & SCleric Quintet 4 - The Fallen Fortress       \\ 
2  & 20,000 Leagues Under the Sea                    & 46 & Shadowdale                                    \\ 
3  & Alice in Wonderland                             & 47 & Spellfire                                     \\ 
4  & Beautiful and the Damned                        & 48 & Star Wars-Dark Force Rising                   \\ 
5  & Bible                                           & 49 & Star Wars-Heir to the Empire                  \\ 
6  & Breakfast at Tiffanys                           & 50 & Star Wars-The Last Command                    \\ 
7  & Clancy Tom - Patriot Games                      & 51 & Tantras                                       \\ 
8  & Clancy Tom - Red Storm Rising                   & 52 & Test Of The Twins                             \\ 
9  & Clarke Arthur C - 3001 The Final Odissey        & 53 & The Age Of Innocence                          \\ 
10 & Cleric Quintet 1 - Canticle                     & 54 & THE Catcher In The Rye                        \\ 
11 & Cleric Quintet 2 - In Sylvan Shadows            & 55 & The Fellowship Of The Ring                    \\ 
12 & Cleric Quintet 3 - Night Masks                  & 56 & The Great Gatsby                              \\ 
13 & Crown of Fire                                   & 57 & The Legend Of Huma                            \\ 
14 & Crucible - The Trial Of Cyric The Mad           & 58 & The little Prince                             \\ 
15 & Dragon lance Preludes 2 vol 2 - Flint the King  & 59 & The Lone Drow                                 \\ 
16 & Dragons of Autumn Twilight                      & 60 & The Return Of The King                        \\ 
17 & Dragons of Spring Dawning                       & 61 & The Second Generation                         \\ 
18 & Dragons of Summer Flame                         & 62 & The Thousand Orcs                             \\ 
19 & Dragons of Winter Night                         & 63 & The Two Swords                                \\ 
20 & Dragonwall                                      & 64 & The Two Towers                                \\ 
21 & Earth's Children 01 - The Clan of the Cave Bear & 65 & The Wheel of Time 01 - Eye of the world       \\ 
22 & Earth's Children 02 - The Valley of Horses      & 66 & The Wheel of Time 02 - The Great Hunt         \\ 
23 & Earth's Children 03 - The Mammoth Hunters       & 67 & The Wheel of Time 03 - The Dragon Reborn      \\ 
24 & Earth's Children 04 - Plains Of Passage         & 68 & The Wheel of Time 04 - The Shadow Rising      \\ 
25 & Earth's Children 05 - The Shelters Of Stone     & 69 & The Wheel of Time 05 - The Fires of Heaven    \\ 
26 & Frank Herbert - Children of Dune                & 70 & The Wheel of Time 06 - Lord of Chaos          \\ 
27 & Frank Herbert - Dune Messiah                    & 71 & The Wheel of Time 07 - A Crown of Swords      \\ 
28 & Frank Herbert - Dune                            & 72 & The Wheel of Time 08 - The Path of Daggers    \\ 
29 & Hamlet                                          & 73 & The Wheel of Time 09 - Winters Heart          \\ 
30 & Harry Potter 1 - Sorcerer's Stone               & 74 & The Wheel of Time 10 - Crossroads of Twilight \\ 
31 & Harry Potter 2 - Chamber of Secrets             & 75 & The Wheel of Time 11 - Knife of Dreams        \\ 
32 & Harry Potter 3 - The Prisoner Of Azkaban        & 76 & The Wheel of Time Prelude - New Spring        \\ 
33 & Harry Potter 4 - The Goblet Of Fire             & 77 & Time Of The Twins                             \\ 
34 & Harry Potter 5 - Order of the Phoenix           & 78 & To Kill a Mockingbird                         \\ 
35 & Harry Potter 6 - The Half Blood Prince          & 79 & The Tipping Point                             \\ 
36 & Harry Potter 7 - Deathly Hollows                & 80 & War Of The Twins                              \\ 
37 & Horselords                                      & 81 & Washington Square                             \\ 
38 & Maggie a girl of the streets                    & 82 & Waterdeep                                     \\ 
39 & Other half lives                                & 83 & {[}Chronicles Of Prydain 1{]} Book of Three   \\ 
40 & Pii                                             & 84 & {[}Chronicles Of Prydain 2{]} Black Cauldron  \\ 
41 & Pride and Prejudice                             & 85 & {[}Chronicles Of Prydain 3{]} Castle Of Llyr  \\ 
42 & Prince of Lies                                  & 86 & {[}Chronicles Of Prydain 4{]} Taran Wanderer  \\ 
43 & Robert Jordan - The Strike at Shayol Ghul       & 87 & {[}Chronicles Of Prydain 5{]} High King       \\ 
44 & Robinson Crusoe                                 &    &                                               \\ \hline
\end{tabular}
\caption{The book list of Books API.}
\label{tab:bookList}
\end{table*}

==> defaultCI-full.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{l|lllllll|lll}
\hline
\multicolumn{1}{c|}{\textbf{}} &
   &
  \multicolumn{6}{c|}{\textbf{Items Distribution}} &
  \multicolumn{3}{c}{\textbf{Categories Distribution}} \\ \hline
\multirow{6}{*}{\textbf{PiXi}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Books}}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
  \multicolumn{1}{c}{} &
  22 &
  28 &
  \multicolumn{1}{l|}{43} &
  0 &
  0 &
  0 &
  26 &
  14 &
  22 \\
 &
  \multirow{2}{*}{\textbf{Movies}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
   &
  20 &
  22 &
  \multicolumn{1}{l|}{69} &
  6 &
  0 &
  29 &
  30 &
  17 &
  26 \\
 &
  \multirow{2}{*}{\textbf{Images}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
   &
  30 &
  11 &
  \multicolumn{1}{l|}{19} &
  5 &
  14 &
  59 &
  26 &
  15 &
  35 \\ \hline
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}PiXi-Hints\end{tabular}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Books}}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
  \multicolumn{1}{c}{} &
  18 &
  6 &
  \multicolumn{1}{l|}{14} &
  1 &
  0 &
  0 &
  30 &
  6 &
  19 \\
 &
  \multirow{2}{*}{\textbf{Movies}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
   &
  20 &
  19 &
  \multicolumn{1}{l|}{76} &
  9 &
  11 &
  71 &
  29 &
  12 &
  29 \\
 &
  \multirow{2}{*}{\textbf{Images}} &
  Suggested &
  ASA &
  \multicolumn{1}{l|}{TSA} &
  Independent &
  ASA &
  TSA &
  Suggested &
  Accepted &
  Total \\
 &
   &
  33 &
  19 &
  \multicolumn{1}{l|}{29} &
  3 &
  14 &
  27 &
  25 &
  15 &
  36 \\ \hline
\end{tabular}
\caption{Items and categories distribution for both PiXi and PiXi-Hints. The term ``Suggested'' refers to users who selected items/categories recommended by the system, while ``Independent'' refers to users who chose items based on their own preference without relying on the system's suggestions.}
\label{tab:defaultI}
\end{table*}

==> hintsRequest.tex <==
\begin{table}[]
\centering
\begin{tabular}{lllll}
\textbf{\begin{tabular}[c]{@{}l@{}}Hints\\ requested\end{tabular}} & \multicolumn{3}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Successful \\ recall\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Unsuccessful \\ recall\end{tabular}} \\ \hline
\textbf{}                                                          & 1 word & 2 words & 3 words & \textbf{}                                                                                 \\ \hline
5/9                                                                & 0/9           & 0/4                 & 0/4                                       & 7/9                                                                                      
\end{tabular}
\caption{PiXi hints request rates}
\label{tab:hintsRequest}
\end{table}

==> invalid.tex <==
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
\textbf{Category} & \textbf{Count} \\ \hline
\begin{tabular}[c]{@{}l@{}}Very vulnerable and predicable passwords\end{tabular}          & 58  \\
\begin{tabular}[c]{@{}l@{}}Identical passwords from robots or the same workers\\ \end{tabular} & 193 \\ \hline
\textbf{Total}    & 251            \\ \hline
\end{tabular}
\caption{The password summary of all the invalid users.}
\label{tab:invalidList}
\end{table}

==> loginTime.tex <==
\begin{table}[]
\centering
\begin{tabular}{llll}
\hline
               & \textbf{Mean} & \textbf{N} & \textbf{Std. Deviation} \\ \hline
\textbf{Control}     & 17.28            & 10         & 8.23                      \\
\textbf{PiXi}     & 42.44            & 9         & 26.54                      \\
\textbf{PiXi-Hints}    & 157.99           & 12        & 145.26                     \\
\textbf{Total} & 70.56            & 31         & 102.95                      \\ \hline
\end{tabular}
\caption{Mean login time across the three conditions}
\label{tab:mean-login}
\end{table}

==> passwordLength.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
               & \textbf{Mean} & \textbf{N} & \textbf{Std. Deviation} \\ \hline
\textbf{Control}     & 9.35            & 71         & 1.73                      \\
\textbf{PiXi}     & 10.87            & 83         & 4.38                      \\
\textbf{PiXi-Hints}    & 11.42           & 84        & 4.01                     \\ \hline
\textbf{Total} & 10.61            & 238         & 3.73                      \\ \hline
\end{tabular}
\caption{Mean password length across the three conditions.}
\label{tab:mean-length}
\end{table}

==> passwordScore.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
               & \textbf{Mean} & \textbf{N} & \textbf{Std. Deviation} \\ \hline
\textbf{Control}     & 1.83            & 71         & 1.04                      \\
\textbf{PiXi}     & 2.16            & 83         & 1.02                      \\
\textbf{PiXi-Hints}    & 2.31           & 84        & 1.17                     \\ \hline
\textbf{Total} & 2.11            & 238         & 1.09                      \\ \hline
\end{tabular}
\caption{Mean password score across the three conditions.}
\label{tab:mean-score}
\end{table}

==> popWordsP+PH.tex <==
\begin{table*}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllllllllll}
\hline
\textbf{Rank} & \textbf{Word} & \textbf{Category} & \textbf{F.} & \textbf{Rank} & \textbf{Word} & \textbf{Category} & \textbf{F.} & \textbf{Rank} & \textbf{Word} & \textbf{Category} & \textbf{F.} \\ \hline
1 & Adam & Movies, Books & \multicolumn{1}{l|}{5} & 19 & coronavirus & Movies,Images & \multicolumn{1}{l|}{2} & 37 & money & Images & 2 \\
2 & green & Images & \multicolumn{1}{l|}{5} & 20 & data & Images & \multicolumn{1}{l|}{2} & 38 & pattern & Images,Books & 2 \\
3 & nature & Movies, Images & \multicolumn{1}{l|}{5} & 21 & deadly & Books & \multicolumn{1}{l|}{2} & 39 & pc & Images & 2 \\
4 & family & Movies & \multicolumn{1}{l|}{4} & 22 & down & Movies,Books & \multicolumn{1}{l|}{2} & 40 & people & Images & 2 \\
5 & world & Movies,Images & \multicolumn{1}{l|}{4} & 23 & Drizzt & Books & \multicolumn{1}{l|}{2} & 41 & person & Images & 2 \\
6 & and & Movies, Books & \multicolumn{1}{l|}{3} & 24 & egg & Movies,Images & \multicolumn{1}{l|}{2} & 42 & phone & Images & 2 \\
7 & flower & Images & \multicolumn{1}{l|}{3} & 25 & escape & Movies & \multicolumn{1}{l|}{2} & 43 & plant & Images & 2 \\
8 & grey & Images & \multicolumn{1}{l|}{3} & 26 & evening & Movies & \multicolumn{1}{l|}{2} & 44 & safe & Movies,Images & 2 \\
9 & happy & Images & \multicolumn{1}{l|}{3} & 27 & eye & Images & \multicolumn{1}{l|}{2} & 45 & scifi & Movies & 2 \\
10 & human & Images & \multicolumn{1}{l|}{3} & 28 & face & Images & \multicolumn{1}{l|}{2} & 46 & seats & Movies,Books & 2 \\
11 & story & Movies & \multicolumn{1}{l|}{3} & 29 & food & Images & \multicolumn{1}{l|}{2} & 47 & sky & Images & 2 \\
12 & tree & Images & \multicolumn{1}{l|}{3} & 30 & friends & Movies & \multicolumn{1}{l|}{2} & 48 & Strange & Movies,Books & 2 \\
13 & trouble & Movies,Books & \multicolumn{1}{l|}{3} & 31 & girl & Images & \multicolumn{1}{l|}{2} & 49 & unique & Movies & 2 \\
14 & united states & Images & \multicolumn{1}{l|}{3} & 32 & hand & Images & \multicolumn{1}{l|}{2} & 50 & usa & Images & 2 \\
15 & beach & Movies,Images & \multicolumn{1}{l|}{2} & 33 & Lando & Books & \multicolumn{1}{l|}{2} & 51 & Vietnam & Movies,Images & 2 \\
16 & blue & Images & \multicolumn{1}{l|}{2} & 34 & leaf & Images & \multicolumn{1}{l|}{2} & 52 & water & Images & 2 \\
17 & brown & Images & \multicolumn{1}{l|}{2} & 35 & Merry & Books & \multicolumn{1}{l|}{2} & 53 & weapons & Books & 2 \\
18 & business & Movies & \multicolumn{1}{l|}{2} & 36 & middle & Movies,Books & \multicolumn{1}{l|}{2} &  &  &  &  \\ \hline
\end{tabular}
}
\caption{The overall most popular words (used more than once) across PiXi and PiXi-Hints.}
\label{tab:most-freq-w-pph}
\end{table*}

==> popWordsP.tex <==
\begin{table*}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll|lll|llllll}
\hline
\multicolumn{3}{c|}{\textbf{Books}} & \multicolumn{3}{c|}{\textbf{Movies}} & \multicolumn{6}{c}{\textbf{Images}} \\ \hline
\textbf{Rank} & \textbf{Word} & \textbf{F.} & \textbf{Rank} & \textbf{Word} & \textbf{F.} & \textbf{Rank} & \textbf{Word} & \multicolumn{1}{l|}{\textbf{F.}} & \textbf{Rank} & \textbf{Word} & \textbf{F.} \\ \hline
1 & deadly & 2/123 & 1 & Adam & 4/165 & 1 & green & \multicolumn{1}{l|}{5/213} & 13 & food & 2/213 \\
2 & Lando & 2/123 & 2 & family & 4/165 & 2 & nature & \multicolumn{1}{l|}{4/213} & 14 & girl & 2/213 \\
3 & Merry & 2/123 & 3 & and & 2/165 & 3 & flower & \multicolumn{1}{l|}{3/213} & 15 & hand & 2/213 \\
4 & weapons & 2/123 & 4 & business & 2/165 & 4 & grey & \multicolumn{1}{l|}{3/213} & 16 & leaf & 2/213 \\
 &  &  & 5 & escape & 2/165 & 5 & happy & \multicolumn{1}{l|}{3/213} & 17 & money & 2/213 \\
 &  &  & 6 & evening & 2/165 & 6 & human & \multicolumn{1}{l|}{3/213} & 18 & pc & 2/213 \\
 &  &  & 7 & friends & 2/165 & 7 & tree & \multicolumn{1}{l|}{3/213} & 19 & people & 2/213 \\
 &  &  & 8 & scifi & 2/165 & 8 & united states & \multicolumn{1}{l|}{3/213} & 20 & phone & 2/213 \\
 &  &  & 9 & story & 2/165 & 9 & blue & \multicolumn{1}{l|}{2/213} & 21 & plant & 2/213 \\
 &  &  & 10 & trouble & 2/165 & 10 & brown & \multicolumn{1}{l|}{2/213} & 22 & sky & 2/213 \\
 &  &  & 11 & unique & 2/165 & 11 & data & \multicolumn{1}{l|}{2/213} & 23 & usa & 2/213 \\
 &  &  & 12 & world & 2/165 & 12 & face & \multicolumn{1}{l|}{2/213} & 24 & water & 2/213 \\
 &  &  &  &  &  &  &  & \multicolumn{1}{l|}{} & 25 & wood & 2/213 \\ \hline
\end{tabular}
}
\caption{The most popular words (used more than once) for each category across PiXi and PiXi-Hints.}
\label{tab:most-freq-w-p}
\end{table*}

==> popWordsPH.tex <==
\begin{table*}[]
\centering
\begin{tabular}{rrrrrrrrr}
\hline
\multicolumn{9}{c}{\textbf{PiXi-Hints}}                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{3}{c|}{\textbf{Books}}                                                                                            & \multicolumn{3}{c|}{\textbf{Movies}}                                                                                           & \multicolumn{3}{l}{\textbf{Images}}                                                                       \\ \hline
\textbf{Rank} & \textbf{Word} & \multicolumn{1}{r|}{\textbf{\begin{tabular}[c]{@{}r@{}}\% Relative \\ Frequency\end{tabular}}} & \textbf{Rank} & \textbf{Word} & \multicolumn{1}{r|}{\textbf{\begin{tabular}[c]{@{}r@{}}\% Relative \\ Frequency\end{tabular}}} & \textbf{Rank} & \textbf{Word} & \textbf{\begin{tabular}[c]{@{}r@{}}\% Relative \\ Frequency\end{tabular}} \\ \hline
1             & Lando      & \multicolumn{1}{r|}{2/501 (0.004%)}                                                                   & 1             & family            & \multicolumn{1}{r|}{3/501 (0.006%)}                                                                   & 1             & happy          & 3/501 (0.006%)                                                                   \\ 
2             & living      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 2             & Adam            & \multicolumn{1}{r|}{2/501 (0.004%)}                                                                   & 2             & data          & 2/501 (0.004%)                                                                   \\ 
3             & look      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 3             & friends            & \multicolumn{1}{r|}{2/501 (0.004%)}                                                                   & 3             & tree          & 2/501 (0.004%)                                                                   \\ 
4             & Merry      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 4             & unique            & \multicolumn{1}{r|}{2/501 (0.004%)}                                                                   & 4             & brown          & 2/501 (0.004%)                                                                   \\ 
5             & Nautilus      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 5             & Village            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 5             & human          & 2/501 (0.004%)                                                                   \\ 
6             & Obould      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 6             & Wagstaff            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 6             & flower          & 2/501 (0.004%)                                                                   \\ 
7             & of      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 7             & zombie            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 7             & girl          & 2/501 (0.004%)                                                                   \\ 
8             & painful      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 8             & about            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 8             & nature          & 2/501 (0.004%)                                                                   \\ 
9             & Potter      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 9             & Adam            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 9             & people          & 2/501 (0.004%)                                                                   \\ 
10             & pushing      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 10             & adapting            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 10             & person          & 2/501 (0.004%)                                                                   \\ 
11             & Russian      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 11             & alive            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 11             & green          & 2/501 (0.004%)                                                                   \\ 
12             & silvery      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 12             & and            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 12             & hand          & 2/501 (0.004%)                                                                   \\ 
13             & sink      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 13             & apocalypse            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 13             & phone          & 2/501 (0.004%)                                                                   \\ 
14             & the      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 14             & Bam            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 14             & pc          & 2/501 (0.004%)                                                                   \\ 
15             & tilgar      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 15             & battles            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 15             & grey          & 2/501 (0.004%)                                                                   \\ 
16             & troubled      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 16             & beach            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 16             & green          & 2/501 (0.004%)                                                                   \\ 
17             & vanquisher      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 17             & bizarre            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 17             & united states          & 2/501 (0.004%)                                                                   \\ 
18             & Voldemorts      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 18             & breaking            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 18             & violent          & 1/501 (0.002%)                                                                   \\ 
19             & Wicked      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 19             & civilization            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 19             & water          & 1/501 (0.002%)                                                                   \\ 
20             & wizard      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 20             & Comedian            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 20             & white          & 1/501 (0.002%)                                                                   \\ 
21             & and      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 21             & couples            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 21             & woman          & 1/501 (0.002%)                                                                   \\ 
22             & beamed      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 22             & curtains            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 22             & yellow          & 1/501 (0.002%)                                                                   \\ 
23             & bedroom      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 23             & down            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 23             & grey          & 1/501 (0.002%)                                                                   \\ 
24             & boldness      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 24             & eggs            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 24             & hike          & 1/501 (0.002%)                                                                   \\ 
25             & Coruscant      & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 25             & escape            & \multicolumn{1}{r|}{1/501 (0.002%)}                                                                   & 25             & honest          & 1/501 (0.002%)                                                                   \\ 
\hline
\end{tabular}

\caption{Most frequent words for each category in PiXi-Hints}
\label{tab:most-freq-w-ph}
\end{table*}

==> registerTime.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
               & \textbf{Mean} & \textbf{N} & \textbf{Std. Deviation} \\ \hline
\textbf{Control}     & 49.61            & 71         & 59.71                      \\
\textbf{PiXi}     & 208.63            & 83         & 281.25                      \\
\textbf{PiXi-Hints}    & 249.85           & 84        & 240.44                     \\
\textbf{Total} & 175.74            & 238         & 236.13                      \\ \hline
\end{tabular}
\caption{Mean register time across the three conditions.}
\label{tab:mean-register}
\end{table}

==> seeds.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{lll}
\hline
\textbf{No.} & \textbf{Formula}                                                                                          & \textbf{Description}                                                                                                                                                                    \\ \hline
1            & \begin{tabular}[c]{@{}l@{}}CategorySeed = \\ Math.seedrandom{[}Amazon MTurk ID + Category{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}When generate a seed, the category is \\ added to make sure the seed is different \\ for the same user when she choose a \\ different category.\end{tabular} \\ \hline
2            & \begin{tabular}[c]{@{}l@{}}CategoryKeyword = \\ BookList{[}CategorySeed{]}\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}A category keyword is randomly \\ selected from a English word list. {[}{]}.\end{tabular}                                                                   \\ \hline
3            & \begin{tabular}[c]{@{}l@{}}DefaultCategoryItems = \\ APIRequest{[}CategoryKeyword{]} *20\end{tabular}     & \begin{tabular}[c]{@{}l@{}}The default 20 random items are \\ fetched from the corresponding  API.\end{tabular}                                                                     \\ \hline
\end{tabular}
\caption{Seed Generating Algorithm \#1}
\label{tab:SGA1}
\end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{lll}
\hline
\textbf{No.} & \textbf{Formula}                                                                                                          & \textbf{Description}                                                                                                                          \\ \hline
1            & \begin{tabular}[c]{@{}l@{}}KeywordSeed \\ = {[}Amazon MTurk ID{]} + \\ {[}Category{]} + {[}Search keyword{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}A new seed is generated by adding a new element \\ "Search keyword" when the user use the search bar.\end{tabular} \\ \hline
2            & \begin{tabular}[c]{@{}l@{}}SearchedCategoryItems = \\ APIRequest{[}SearchSeed{]} *20\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}20 random items are fetched using \\ the new seed from the corresponding API.\end{tabular}                  \\ \hline
\end{tabular}
\caption{Seed Generating Algorithm \#2}
\label{tab:SGA2}
\end{table*}

==> uniqueWordsRef.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{rrr}
\hline
\multicolumn{3}{c}{\textbf{Unique words references (Books)}}                                                                   \\ \hline
\multicolumn{1}{l}{\textbf{Title}}                         & \multicolumn{1}{r}{\textbf{Total Words}} & \textbf{Unique Words} \\ 
\multicolumn{1}{l}{Bible (KJV)}                            & \multicolumn{1}{r}{857,116}              & 13,076                \\ 
\multicolumn{1}{l}{Breakfast at Tiffanys}                  & \multicolumn{1}{r}{27,790}               & 4,893                 \\ 
\multicolumn{1}{l}{The Wheel of Time 11 - Knife of Dreams} & \multicolumn{1}{r}{328,633}              & 13,844                \\ 
\multicolumn{1}{l}{Harry Potter 7 - Deathly Hollows}       & \multicolumn{1}{r}{200,888}              & 11,411                \\ 
\multicolumn{1}{l}{The Two Towers}                         & \multicolumn{1}{r}{156,379}              & 19,622                \\ \hline
\end{tabular}
\caption{Unique Words Reference List}
\label{tab:uniqueWordsRef}
\end{table*}
